Search for Single Top Quark Production Using Likelihood Discriminants at D0 in Run II

We present an improved search for single top quarks in two production modes, s-channel (tb) and t-channel (tqb). The search is performed in the electron+jets and muon+jets decay channels, with one or more b-tagged jets, on nearly 370 pb^{-1} of D0 Run II data collected between August 2002 and October 2004. Impact-parameter based b-quark tagging is used to select signal-like events. We use a likelihood discriminant method to separate signals from backgrounds. The resulting expected/observed 95% confidence level upper limits on the single top quark production cross sections are 3.3/5.0pb (s-channel) and 4.3/4.4pb (t-channel).

==> tex/acknowledgement_paragraph_r2.tex <==
% acknowledgement_paragraph_r2.tex                5/17/05
%
We thank the staffs at Fermilab and collaborating institutions, 
and acknowledge support from the 
DOE and NSF (USA);
CEA and CNRS/IN2P3 (France);
FASI, Rosatom and RFBR (Russia);
CAPES, CNPq, FAPERJ, FAPESP and FUNDUNESP (Brazil);
DAE and DST (India);
Colciencias (Colombia);
CONACyT (Mexico);
KRF (Korea);
CONICET and UBACyT (Argentina);
FOM (The Netherlands);
PPARC (United Kingdom);
MSMT (Czech Republic);
CRC Program, CFI, NSERC and WestGrid Project (Canada);
BMBF and DFG (Germany);
SFI (Ireland);
Research Corporation,
Alexander von Humboldt Foundation,
and the Marie Curie Program.
%


==> tex/btagging.tex <==
\section{Lifetime b-tagging}
\vspace{-0.15cm}
\begin{figure}[!ht]
\includegraphics[width=0.48\textwidth]{figures/JLIP_eff_0.eps}
\includegraphics[width=0.48\textwidth]{figures/JLIP_eff_1.eps}
\includegraphics[width=0.48\textwidth]{figures/JLIP_eff_2.eps}
\includegraphics[width=0.48\textwidth]{figures/JLIP_eff_3.eps}
\caption[]{JLIP $b$-tagging efficiencies in the electron channel data as a function of jet $p_T$ (at $\eta = 0.5$) and jet $\eta$ (at $p_T$ = 60~GeV) for the Loose (red curve) and
Tight (blue curve) probability cuts. These curves include the
taggability efficiency. The first row corresponds to the $b$-jets tagging efficiency and the second to the light jet mistag rate. The dashed curves correspond to the total $\pm1\sigma$ systematic error bands.}
\label{fig-jlipeff}
\vspace{-0.2cm}
\end{figure}
The event selection requires at least one $b$-tagged jet. Prior to tagging we require
calorimeter jets to be taggable i.e. matched to a track jet. We are using the Jet LIfetime Probability (JLIP) algorithm of the
\dzero Collaboration~\cite{SebJLIP}. It uses the signed impact parameter of tracks (representing the distance of closest approach of a track w.r.t
the primary vertex)  within a jet to compute a probability for
the jet to originate from the primary vertex. Heavy  quark jets are expected to have low values for the JLIP probability.
Jets are tagged if their JLIP probability is smaller than a given cut. The probability distribution is expected to be
flat for light jets and therefore the cut value gives approximately the mistag rate. In the analysis we are using two different
probability cuts : Tight ($P_{JLIP}<0.3\%$) and Loose ($P_{JLIP}<1.0\%$). Efficiencies (including taggability) for each probability
cuts are
given in Fig.~\ref{fig-jlipeff}.\\
The dataset is splitted into two orthogonal tagging schemes. The ``single tag" sample corresponds to events containing exactly one Tight and no extra Loose $b$-tagged jet. The ``double tag" sample is associated to events with at least one Tight and another Loose $b$-tagged jets.



==> tex/dataset.tex <==
\section{Data and Simulated samples}
\vspace{-0.15cm}
The analysis partitioned by decay mode, in electron and muon channels, is based on Run~II data recorded between August 2002 and October 2004.
The integrated luminosity is $366\pm 24 \; $pb$^{-1}$ for the electron channel and $363\pm 24\; $pb$^{-1}$ for
 the muon channel. The different luminosities are due to different data quality requirements.
The Monte Carlo samples for
$t\bar{t}\rightarrow l\nu b jj \bar{b}$ (lepton+jet), $t\bar{t}\rightarrow l\nu b l\nu \bar{b}$ (dileptons),
$W$+jets ($Wbb$ and $Wjj$) and diboson ($WW\rightarrow l \nu jj$, $WZ\rightarrow l\nu jj$) processes were
generated using Alpgen~\cite{Mangano:2002ea} for hard interaction matrix elements calculations (at leading order) coupled to Pythia~\cite{pythiaref}
for Initial State Radiation, Final State Radiation, hadronization and fragmentation. Single top quark signal samples were produced with a
modified version of CompHep \cite{comphepref} interfaced to Pythia in order to reproduce the  next-to-leading order kinematic
distributions of the decay particles in the $s$-channel and $t$-channel.
The Monte Carlo samples are processed
with  the full Geant~\cite{geantref} simulation of the \dzero detector and passed through the \dzero event reconstruction
program. The resulting lepton and jet energies are smeared to reproduce the resolutions observed in data.



==> tex/eventreco.tex <==
\section{Event Reconstruction And Selection}
\vspace{-0.15cm}
\label{select}
The events are selected by requiring  simple cuts on reconstructed objects.
The event primary vertex must have at least 3 tracks and a position along the beam axis not greater
than 60~cm from $z = 0$.
Jets are reconstructed using the standard \dzero cone algorithm ($\Delta R<0.5$). For jets within the trigger system acceptance, a
confirmation of the jet at Level 1 is required.
Each event is required to have between  two and four  good jets with a leading jet
satisfying $p_T>25$~GeV and $|\eta|<2.5$. Other good jets should have $p_T>15$~GeV and $|\eta|<3.4$. Jet energy is corrected for
out-of-cone showering, calorimeter non uniformity, and the difference in calorimeter response between electrons and pions.
Electrons are reconstructed using information from both the calorimeter and the central tracker. Muons are reconstructed using
information from the muon spectrometer with a detector pseudorapidity acceptance $|\eta^{det}|<2$.
The event must contain only one isolated lepton with $p_T>15$~GeV. For the electron channel, only electrons in
the central part of the calorimeter ($|\eta^{det}|<1.1$) are considered. Both muon and electron must be well matched to a track.
For the muon selection, among additional requirements muon candidates within any jet cone (i.e. $\Delta R(\mu,jet)<0.5$) are rejected.
In order to account for the presence of a neutrino, some constraints are applied on
the  missing transverse energy (\MET) (corrected for the presence of electrons, muons and jets in the event).  We require
$\MET^{JES}>15$~GeV and $15<\MET<200$~GeV, where $\MET^{JES}$  is the missing transverse energy with jet energy scale correction
applied and \MET has also corrections for the energy of an isolated muon. QCD multijet events where \MET$\;$ results from misreconstructed objects (jets or electrons) are
rejected by imposing cuts in the planes $\MET-\Delta\phi({\rm lepton},\MET)$ and $\MET-\Delta\phi(jet,\MET)$.
Finally, at least one of the good jets must satisfy the Tight $b$-tagging criteria (see next Section).



==> tex/signature.tex <==
\section{Signal signature}
\vspace{-0.15cm}
The top quark is the heaviest known particle. Its large mass and small decay length confer it unique properties. 
It decays before hadronization can occur, and spin information is
preserved in the decay products, which leads to angular correlations in
the final state objects that are characteristic for this signal.
This analysis focuses on the final state
topology where the top quark decays into a $b$ quark and a $W$ boson, which
subsequently decays leptonically ($W\rightarrow e\nu ,\mu\nu$). The signal signature consists of an
isolated high
transverse momentum lepton (electron or muon), significant missing transverse energy carried out by the neutrino and two or
three high transverse momenta jets including at least one $b$ jet. The largest backgrounds with a
similar topology are the associated production of a $W$ boson with jets ($W$+jets) and  $t{\bar t}$ production.
Additional multijet background comes from events containing a fake isolated lepton (jet identified as electron or muon from
$B$ hadron decays or decays in flight) associated with hadronic jets. Smaller contributions from diboson ($WW$,$WZ$) events are also considered.



==> tex/systematics.tex <==
\section{Systematic uncertainties}
\vspace{-0.15cm}
Systematic uncertainties on the yields are evaluated separately for electron and muon channels for each $b$-tagging scheme. Sources of systematics and their range values
are summarized in Table~\ref{tab-systM} for Monte Carlo yields ($t\bar{t}$, diboson) and in Table~\ref{tab-systD} for yields normalized to data (multijet and $W$+jets).

\begin{table}[h]
\begin{center}
\begin{minipage}{0.485\textwidth}
\begin{ruledtabular}
\begin{tabular}{lc}
\multicolumn{2}{c}{\underline{Systematics uncertainties (\%)}}\\
& Single (Double) Tag  \\
\hline
Luminosity & 6.5 \\
Cross section				& 2($$WW)-18($t\bar{t}$)\\
Branching fraction			& 2\\

Primary vertex reconstruction		&2\\
Electron identification 	&4\\
Muon identification 		&5\\
Jet identification 		&1-4\\
Jet energy scale			&1-5\\
Jet energy resolution			&1\\
Jet fragmentation			&5\\
Trigger modeling			&2-7\\
b-tagging modeling			&6 (17)\\
Samples statistics			&1\\
\end{tabular}
\end{ruledtabular}
\vspace{-0.1in}
\caption[tab-systM]{Averaged systematic uncertainties for Monte Carlo estimated yields.}
\label{tab-systM}
\end{minipage}
$\quad$
\begin{minipage}{0.485\textwidth}
\begin{ruledtabular}
\begin{tabular}{lc}
 \multicolumn{2}{c}{\underline{Systematics uncertainties (\%)}}\\
& Single (Double) Tag \\
\hline
Data normalization			&5-15\\
b-tagging modeling ($W$+jets only)	&9 (15)\\
Samples statistics			&3 (2-17)\\
\end{tabular}
\end{ruledtabular}
\begin{tabular}{lc}
&\\
&\\
&\\
&\\
&\\
&\\
&\\
&\\
&\\
&\\
\end{tabular}
\vspace{-0.1in}
\caption[tab-systD]{Averaged systematic uncertainties for data normalized yields.}
\label{tab-systD}
\end{minipage}
\end{center}
\vspace{-0.7cm}
\end{table}

